Instruction-Guided Autoregressive Neural Network Parameter Generation

Learning to generate neural network parameters conditioned on task descriptions and architecture specifications is pivotal for advancing model adaptability and transfer learning. Existing methods especially those based on diffusion models suffer from limited scalability to large architectures, rigidity in handling varying network depths, and disjointed parameter generation that undermines inter-layer coherence. In this work, we propose IGPG (Instruction Guided Parameter Generation), an autoregressive framework that unifies parameter synthesis across diverse tasks and architectures. IGPG leverages a VQ-VAE and an autoregressive model to generate neural network parameters, conditioned on task instructions, dataset, and architecture details. By autoregressively generating neural network weights' tokens, IGPG ensures inter-layer coherence and enables efficient adaptation across models and datasets. Operating at the token level, IGPG effectively captures complex parameter distributions aggregated from a broad spectrum of pretrained models. Extensive experiments on multiple vision datasets demonstrate that IGPG consolidates diverse pretrained models into a single, flexible generative framework. The synthesized parameters achieve competitive or superior performance relative to state-of-the-art methods, especially in terms of scalability and efficiency when applied to large architectures. These results underscore ICPG potential as a powerful tool for pretrained weight retrieval, model selection, and rapid task-specific fine-tuning.

==> plots/cross_dataset.tex <==


\begin{figure}[t!]
    \centering
    \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.0\textwidth]{img/cross_plot_mnist_fig.pdf}
            \caption{MNIST}
            \label{figmnist}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.0\textwidth]{img/cross_plot_svhn_fig.pdf}
            \caption{SVHN}
            \label{figsvhn}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width= 1.0\textwidth]{img/cross_plot_cifar-10_fig.pdf}
            \caption{CIFAR-10}
            \label{figcifar}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
	\includegraphics[width=1.0\textwidth]{img/cross_plot_stl-10_fig.pdf}
        \caption{STL-10}
         \label{figstl}
    \end{subfigure}
	% \vspace{-0.13in}
        \caption{The assessment of cross-dataset transfer learning begins by initializing the model with sampled weights, which is then fine-tuned over 25 epochs. The model's performance is evaluated against three benchmarks: the baseline model, a model trained from scratch with random weight initialization, and pretrained models.}
        \label{fig:cross}
	\vspace{-0.15in}
\end{figure}

==> plots/finetune.tex <==

\begin{figure}[t!]
    \centering
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.0\textwidth]{img/indist_plot_mnist_fig.pdf}
            \caption{MNIST}
            \label{figmnist}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.0\textwidth]{img/indist_plot_svhn_fig.pdf}
            \caption{SVHN}
            \label{figsvhn}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width= 1.0\textwidth]{img/indist_plot_cifar-10_fig.pdf}
            \caption{CIFAR-10}
            \label{figcifar}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
	\includegraphics[width=1.0\textwidth]{img/indist_plot_stl-10_fig.pdf}
        \caption{STL-10}
         \label{figstl}
    \end{subfigure}
	% \vspace{-0.13in}
        \caption{Average accuracy progression during fine-tuning over 25 epochs with sampled weights. The sampled weights are evaluated on the same pre-trained datasets to compare their performance against both the existing method and the original pre-trained model.}
        \label{neuripsevol}
	% \vspace{-0.15in}
\end{figure}

==> plots/unseen_datasets.tex <==


\begin{figure}[t!]
    \centering
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.0\textwidth]{img/unseen_mnist_fig.pdf}
            \caption{MNIST}
            \label{fig:mnist}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=1.0\textwidth]{img/unseen_svhn_fig.pdf}
            \caption{SVHN}
            \label{fig:svhn}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
            \includegraphics[width= 1.0\textwidth]{img/unseen_cifar-10_fig.pdf}
            \caption{CIFAR-10}
            \label{fig:cifar}
    \end{subfigure}
    % \vspace{-0.1in}
     \begin{subfigure}{0.24\linewidth}
	\includegraphics[width=1.0\textwidth]{img/unseen_stl-10_fig.pdf}
        \caption{STL-10}
         \label{fig:stl}
    \end{subfigure}
	% \vspace{-0.13in}
        \caption{Performance evaluation on unseen datasets with HyperVQGAN and HyperCVAE}
        \label{fig:unseen}
	% \vspace{-0.15in}
\end{figure}

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
